End-to-End Object Detection with Transformers

We present a new method that views object detection as a direct set prediction problem. Our approach streamlines the detection pipeline, effectively removing the need for many hand-designed components like a non-maximum suppression procedure or anchor generation that explicitly encode our prior knowledge about the task. The main ingredients of the new framework, called DEtection TRansformer or DETR, are a set-based global loss that forces unique predictions via bipartite matching, and a transformer encoder-decoder architecture. Given a fixed small set of learned object queries, DETR reasons about the relations of the objects and the global image context to directly output the final set of predictions in parallel. The new model is conceptually simple and does not require a specialized library, unlike many other modern detectors. DETR demonstrates accuracy and run-time performance on par with the well-established and highly-optimized Faster RCNN baseline on the challenging COCO object detection dataset. Moreover, DETR can be easily generalized to produce panoptic segmentation in a unified manner. We show that it significantly outperforms competitive baselines. Training code and pretrained models are available at https://github.com/facebookresearch/detr.

==> ablations.tex <==
\subsection{Extended ablation study} 

This section contains the results of ablation experiments referenced from the main text (Section 4.2).

\subsubsection{Importance of positional encoding.}
There are two kinds of positional encoding in our model: spatial 
positional encoding and output positional encoding (object queries).
We experiment with various combinations of fixed and learned encodings for the spatial encodings. The positional encodings are shared between all layers,
and the output encoding (object queries) is always learned. The
results are given in Table~\ref{table:pos_enc}.
The first experiment removes both kinds of positional encoding altogether,
and, interestingly, the model still achieves 
more than 31 AP, losing 6 AP to the baseline.
Then, we add fixed sine spatial positional encoding and output encoding
to the input, as in the original transformer~\cite{Vaswani2017AttentionIA},
and find that this leads to 1.1 AP drop compared to passing positional encoding
at every attention layer. Learned spatial encoding at every attention layers gives
similar results to fixed sine encodings added to inputs.
Surprisingly, we find that removing the positional embeddings of the encoder
only leads to a minor AP drop.
In all cases, encodings are shared between all layers,
and output encoding (object queries) is always learned.
\setlength{\tabcolsep}{0.7em}
\begin{table}[h!]
    \centering\small
    \caption{Results for different positional encodings compared
    to baseline (last row), which has a fixed sine pos. encoding passed
    at every attention layer in both the encoder and decoder.
    Learned embedding is shared in all the layers.
    Not using positional encoding leads to a significant
    drop in AP. Interestingly, passing it in decoder only
    leads to a minor AP drop.\label{table:pos_enc}}
    \begin{tabular}{lcc|cc|cc}
        \toprule
        encoding & encoder & decoder & AP & $\Delta$ & \AP{50} & $\Delta$ \\
        \midrule
        none                & &     
        & 31.0 & -6.4 & 51.6 & -4.8 \\
        sine at input        & \chk & \chk
        & 36.2 & -1.1 & 55.1 & -1.3 \\
        learned at attention & \chk & \chk
        & 36.1 & -1.2 &	55.8 & -0.6 \\
        sine at attention & & \chk
        & 36.8 & -0.5 &	56.2 & -0.1 \\
        sine at attention & \chk & \chk
        & \textbf{37.3} & - & \textbf{56.4} & - \\
        \bottomrule
    \end{tabular}
\end{table}
Interestingly, the model without any positional encoding still achieves 
more than 31 AP, losing 6 AP to the baseline.
The model with absolute encoding added to the input only
loses 1.4 AP vs. baseline. 

\subsubsection{Cost ablations.} 
To evaluate the importance of different parts of the matching cost,
we train several models turning them on and off.
There are two main components to the cost: classification cost and box cost (\ref{eq:bloss}), consisting of GIoU and $\ell_1$ bounding box distance.
The classification cost is essential for training and cannot be turned off,
so we train a model without bounding box distance loss, and a model without the GIoU loss,
setting either $\lambda_{\rm iou}$ or $\lambda_{\rm L1}$ in the cost and in the loss to zero,
and compare with baseline.
Results are presented in Table~\ref{table:cost}.
\setlength{\tabcolsep}{0.7em}
\begin{table}[h!]
    \centering\small
    \caption{Effect of cost parts on AP.
    We train two models turning off box cost and GIoU cost,
    and observe that box cost gives better results on large objects,
    whereas GIoU cost is better on small.
    \detr (last row) combines both costs.
    }
    \begin{tabular}{ccc|cc|cc|ccc}
        \toprule
        class & $\ell_1$ & GIoU & AP & $\Delta$ & \AP{50} & $\Delta$ & \AP{S} & \AP{M} & \AP{L} \\
        \midrule
        \chk & \chk & &
        35.4 & -1.8 & 55.3 & -1.1 & 13.7 &	38.9 &	\textbf{56.4} \\
        \chk & & \chk &
        35.5 & -1.9 & 55.2 & -1.1 & 16.6 &	39.6 &	51.0 \\
        \chk & \chk & \chk &
        \textbf{37.3} & - & \textbf{56.4} & - & \textbf{17.8} &	\textbf{40.5} &	54.3 \\
        \bottomrule
    \end{tabular}
    \label{table:cost}
\end{table}
The GIoU cost shows better results on small objects (+2.9 AP difference),
whereas the bounding box cost improves results on large objects (+5.5 AP difference),
higher than the baseline. We only studied simple ablations of different costs (adding or removing one, and not retuning their weighting every time),
but perhaps other means of combining them could achieve different results.

\iffalse
\setlength{\tabcolsep}{0.7em}
\begin{table}[h!]
    \centering\small
    \begin{tabular}{ccc|cc|cc|ccc}
        \toprule
        class & bbox & GIoU & AP & $\Delta$ & \AP{50} & $\Delta$ & \AP{S} & \AP{M} & \AP{L} \\
        \midrule
        \chk & \chk & &
        35.4 & -1.8 & 55.3 & -1.1 & 13.7 &	38.9 &	\textbf{56.4} \\
        \chk & & \chk &
        35.5 & -1.9 & 55.2 & -1.1 & 16.6 &	39.6 &	51.0 \\
        \chk & \chk & \chk &
        \textbf{37.3} & - & \textbf{56.4} & - & \textbf{17.8} &	\textbf{40.5} &	54.3 \\
        \bottomrule
    \end{tabular}
    \caption{Effect of cost parts on AP.
    We train two models turning off box cost and GIoU cost,
    and observe that box cost gives better results on large objects,
    whereas GIoU cost is better on small.
    Our baseline (last row) combines both costs.
    }
    \label{table:cost}
\end{table}
\setlength{\tabcolsep}{0.5em}
\begin{figure}
\small
\begin{subfigure}[t!]{0.46\textwidth}
    \begin{tabular}{lccc}
        \toprule
        encoding & enc. & dec. & AP \\
        \midrule
        none                & &     
        & 31.0  \\
        sine @ input        & \chk & \chk
        & 36.2  \\
        learned @ attn & \chk & \chk
        & 36.1  \\
        sine @ attn & & \chk
        & 36.8  \\
        sine @ attn & \chk & \chk
        & \textbf{37.3} \\
        \bottomrule
    \end{tabular}
    \caption{Results for different positional encodings compared
    to baseline (last row), which has a fixed sine pos. encoding passed
    at every attention layer in both the encoder and decoder.
    \label{table:pos_enc}}
\end{subfigure}
\begin{subfigure}[t!]{0.52\textwidth}
    \begin{tabular}{cccccc}
        \toprule
        class & bbox & GIoU & AP %
        & \AP{S} %
        & \AP{L} \\
        \midrule
        \chk & \chk & &
        35.4 %
        & 13.7 %
        &	\textbf{56.4} \\
        \chk & & \chk &
        35.5 %
        & 16.6 %
        &	51.0 \\
        \chk & \chk & \chk &
        \textbf{37.3} %
        & \textbf{17.8} %
        &	54.3 \\
        \bottomrule
    \end{tabular}
    \caption{Effect of the parts of the loss on AP.
    We train two models turning off the box cost and the GIoU cost,
    and observe that the box cost gives better results on large objects,
    whereas GIoU cost is better on small.
    Our baseline (last row) combines both costs.
    \label{table:cost}}
\end{subfigure}
    \caption{TODO TODO TODO\label{fig:posencodingandcostablations}}
\end{figure}
\fi


==> background.tex <==
\section{Background}
\label{sec:background}

In this section we briefly describe the transformer architecture~\cite{Vaswani2017AttentionIA}.
We describe our modifications enabling set prediction in sec.~\ref{sec:method}, to which a reader familiar with
transformer architecture can skip directly.

\textit{Multi-head attention} is the core operation of the transformer.
We apply scaled dot-product multi-head attention, defined as:
\[\text{Attention}(\mQ, \mK, \mV) = \text{softmax}(\frac{\mQ\mK^T}{\sqrt{d}})\mV,\]
where $\mQ$, $\mK$ and $\mV$ are input matrices called query, key and value respectively,
and $d$ is number of channels in $\mK$.
In self-attention query, key and value matrices are obtained by projecting
the same input $\mX$ with different weights $W_{q,k,v}$:
$\mQ = \mW_q\mX$, $\mK = \mW_k\mX$, $\mV = \mW_v\mX$.
In inter-attention query is a different input.
Additionally, the multi-head aspect is achieved by doing attention multiple times with different weights on the same
inputs, and concatenating the outputs.

Let's define self-attention for 2D inputs, corresponding to activations of a convolutional network.
In this case input $\mX$ has shape $NHWC$, where $N$ is batch size,
$HW$ is activation height and width, and $C$ is the number of channels.
Query, key and value is then the same matrix, thus the name of the function.
An \textit{attention map} is a product of $\mX$ projected into $\mQ$ and $\mK$ after softmax,
computed for each sample in a minibatch and has $HW\times HW$ shape.
Self-attention thus has ability to `attend' to specific regions in the image, given the whole scene,
and utilize context.
Current region-based detectors lack this ability due to local region-detection relationship assumption.
In decoder inter-attention the size of the attention map computed is $H\times W$.

We adopt a common encoder-decoder architecture.
Encoder consists of multiple multi-head self-attention layers followed by a feed-forward network (FFN, or MLP) and layer normalization:
\begin{align}
    \mQ_\text{MHA} &= \text{layernorm}\Big(\mQ + \text{dropout}\big(\text{Attention}(\mQ, \mK, \mV)
        \big)\Big),\\
    \mQ &= \text{layernorm}(\mQ_\text{MHA} + \text{dropout}(\mW_2\text{relu}(\mW_1\mQ_\text{MHA}))),
    \label{eq:mha}
\end{align}
$\mW_1$ and $\mW_2$ are FFN weights.
We pass CNN activations through a single $1\times1$ convolutional layer and flatten
before feeding it to encoder as $\mQ$, $\mK$ and $\mV$.
Self-attention in encoder allows learning the regions of interest for classifying and localizing the object given the whole image.
Encoder output is called memory, which is fed into decoder together with $N$ query embeddings.
For each query embedding decoder outputs an object, or none, in parallel, as described later.
Decoder constists of multiple self-attention layers on query outputs,
inter-attention between query outputs and encoder memory, followed by FFN.
In inter-attention, $\mK$ and $\mQ$ are query outputs, and $\mV$ is encoder memory.

==> symbolsdef.tex <==
\newcommand{\M}{\mathcal M}
\newcommand{\A}{\mathcal A}
\newcommand{\B}{\mathcal B}
\renewcommand{\O}{\mathcal O}
\renewcommand{\L}{\mathcal L}
\newcommand{\calS}{\mathcal S}
\newcommand{\R}{\mathcal R}
\newcommand{\T}{\mathcal T}
\newcommand{\calP}{\mathcal P}
\newcommand{\X}{\mathcal X}
\newcommand{\Y}{\mathcal Y}
\newcommand{\calE}{\mathcal E}
\newcommand{\parent}{\textsc{par}}
\renewcommand{\Re}{\mathbb{R}}

\DeclareMathOperator*{\Argmax}{Arg\,max}
\DeclareMathOperator*{\Argmin}{Arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\sign}{sign}
\DeclareMathOperator*{\subExp}{subExp}
\DeclareMathOperator*{\subGauss}{subGauss}
\newcommand{\Meq}{\text{eq}}
\DeclareMathOperator*{\Var}{Var}

\newcommand{\ucrl}{{\small\textsc{UCRL}}\xspace}
\newcommand{\ucrlsmdp}{{\small\textsc{UCRL-SMDP}}\xspace}
\newcommand{\sucrl}{{\small\textsc{SUCRL}}\xspace}
\newcommand{\freesucrl}{{\small\textsc{FSUCRL}}\xspace}
\newcommand{\freesucrlA}{{\small\textsc{FSUCRLv1}}\xspace}
\newcommand{\freesucrlB}{{\small\textsc{FSUCRLv2}}\xspace}
\newcommand{\pluginsucrl}{{\small\textsc{Est-SUCRL}}\xspace}
\newcommand{\rmax}{{\small\textsc{RMax}}\xspace}
\newcommand{\rmaxbound}{r_{\max}}
\newcommand{\rmaxsmdp}{{\small\textsc{RMax-SMDP}}\xspace}
\newcommand{\fmdp}{fMDP\xspace}
\newcommand{\abs}{\text{abs}}
\newcommand{\bbeta}{\boldsymbol{\beta}}


\newcommand{\blambda}{\boldsymbol{\lambda}}

\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\wo}[1]{\overline{#1}}
\newcommand{\wb}[1]{\overline{#1}}
